EvoK: Connecting loved ones through Heart Rate sharing

In this work, we present EvoK, a new way of sharing one's heart rate with feedback from their close contacts to alleviate social isolation and loneliness. EvoK consists of a pair of wearable prototype devices (i.e., sender and receiver). The sender is designed as a headband enabling continuous sensing of heart rate with aesthetic designs to maximize social acceptance. The receiver is designed as a wristwatch enabling unobtrusive receiving of the loved one's continuous heart rate with multi-modal notification systems.

==> 6-LimitationsAndFutureWork.tex <==
% \section{Limitation and Future Work}

% \subsection{Limitation}
% % There are a few limitations of our final wearable device. 
% While working with Micro:bit, we realized that the processor is not robust enough to support a quick transmission of accurate heart rates to the receiver. We even experienced a delay in receiving the appropriate heart rate and using corresponding vibration feedback for it. The vibration feedback did not work. So, maybe for future studies, a robust processor to support haptic feedback and white led light. Another limitation was capturing correct heart rates in correspondence with the physical state of the individual. We noticed that even when we exercised, the sensor did not reflect high heart rates. To ensure accurate results, it is suggested to use efficient sensors to capture true heart rate variations. Additionally, the current wearable device does not have the feature to personalize the heart rates for oneself; we currently use the same heart rate ranges for notifications for everyone. Moreover, the device is designed as a basic minimum viable product that could be further beautified by encasing the wires.
% \subsection{Future Work}
% We discuss a few future directions that resulted from our current work. One of the first research directions is to perform a usability study to understand if the present form factor would be used and accepted by the users to share their heart rates. Similarly, to evaluate if the device’s notifications are ambient for users considering their different contexts and scenarios. Future research could also empower the users to customize their heart rates; for instance, what according to their body is a normal heart rate and what is abnormal. This feature would help the users to calibrate the notifications depending on their personal heart rate ranges.

==> 8-Acknowledge.tex <==
\section{Acknowledgments}
We will remove this section for the double-blind review. Once the paper is accepted, we can then acknowledge individuals and organizations who helped with the research significantly.  
% Identification of funding sources and other support, and thanks to
% individuals and groups that assisted in the research and the
% preparation of the work should be included in an acknowledgment
% section, which is placed just before the reference section in your
% document.

% This section has a special environment:
% \begin{verbatim}
%   \begin{acks}
%   ...
%   \end{acks}
% \end{verbatim}
% so that the information contained therein can be more easily collected
% during the article metadata extraction phase, and to ensure
% consistency in the spelling of the section heading.

% Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

% \section{Appendices}

% If your work needs an appendix, add it before the
% ``\verb|\end{document}|'' command at the conclusion of your source
% document.

% Start the appendix with the ``\verb|appendix|'' command:
% \begin{verbatim}
%   \appendix
% \end{verbatim}
% and note that in the appendix, sections are lettered, not
% numbered. This document has two appendices, demonstrating the section
% and subsection identification method.

% \section{SIGCHI Extended Abstracts}

% The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
% not in Word) produces a landscape-orientation formatted article, with
% a wide left margin. Three environments are available for use with the
% ``\verb|sigchi-a|'' template style, and produce formatted output in
% the margin:
% \begin{itemize}
% \item {\verb|sidebar|}:  Place formatted text in the margin.
% \item {\verb|marginfigure|}: Place a figure in the margin.
% \item {\verb|margintable|}: Place a table in the margin.
% \end{itemize}

% %%
% %% The acknowledgments section is defined using the "acks" environment
% %% (and NOT an unnumbered section). This ensures the proper
% %% identification of the section in the article metadata, and the
% %% consistent spelling of the heading.
% \begin{acks}
% To Robert, for the bagels and explaining CMYK and color spaces.
% \end{acks}


